Streaming Video Understanding and Multi-round Interaction with Memory-enhanced Knowledge

Recent advances in Large Language Models (LLMs) have enabled the development of Video-LLMs, advancing multimodal learning by bridging video data with language tasks. However, current video understanding models struggle with processing long video sequences, supporting multi-turn dialogues, and adapting to real-world dynamic scenarios. To address these issues, we propose StreamChat, a training-free framework for streaming video reasoning and conversational interaction. $\StreamChat$ leverages a novel hierarchical memory system to efficiently process and compress video features over extended sequences, enabling real-time, multi-turn dialogue. Our framework incorporates a parallel system scheduling strategy that enhances processing speed and reduces latency, ensuring robust performance in real-world applications. Furthermore, we introduce StreamBench, a versatile benchmark that evaluates streaming video understanding across diverse media types and interactive scenarios, including multi-turn interactions and complex reasoning tasks. Extensive evaluations on StreamBench and other public benchmarks demonstrate that StreamChat significantly outperforms existing state-of-the-art models in terms of accuracy and response times, confirming its effectiveness for streaming video understanding. Code is available at StreamChat: https://github.com/hmxiong/StreamChat.

==> Section/Limitations.tex <==
\section{Limitations and future works}\label{Limitations}
\textbf{Fine-grained Retrieval}:
In order to further improve the performance of the model in online scenarios, we believe that more fine-grained information retrieval is the key. Our retrieval algorithm is still a simple matching method at present, and there is still the possibility of matching errors, which will directly cause the model to go to the wrong memory branch and fail to generate the correct answer.

\textbf{VRAM budget}:
Although our method can achieve compression and storage of video information, the tree-structured storage method is still limited by VRAM as discussed in Sec.~\ref{Ablation}. As the video time increases or the memory parameters change, our method is at risk of exceeding the existing limit.
% We may need to find more efficient or learnable compression methods to solve this problem.
It will be better if we find a more efficient or learnable compression method to solve this problem.

\textbf{Lower Latency}:
To achieve lower latency, closer integration with hardware systems may be necessary to handle larger model parameters and support more efficient inference for a higher volume of user requests. For instance, adopting a more comprehensive multi-modal distributed system or leveraging fast-serving frameworks like SGLang~\cite{zheng2023efficiently} and vLLM~\cite{kwon2023efficient} could significantly enhance performance.
% We think that to achieve lower latency, we may need to work closely with the hardware system to handle larger model parameters and achieve efficient inference for more user requests. For example, a more complete multi-modal distributed system or a fast-serving framework similar to SGLang~\citep{zheng2023efficiently} and vLLM~\citep{kwon2023efficient}.
